Optimized thermoelectric sensitivity measurement for differential thermometry with thermopiles

A novel approach to calibrate the sensitivity of a differential thermometer, consisting of several thermocouples connected in series (thermopile), has been developed. The goal of this method is to increase the accuracy of small temperature difference measurements ($\Delta T \leq 1\:\textrm{K}$), without invoking higher sensor complexity. To this end, a method to determine the optimal temperature difference employed during the differential measurement of thermoelectric sensitivities has been developed. This calibration temperature difference is found at the minimum of combined measurement and linearization error for a given mean temperature. The developed procedure is demonstrated in an illustrative example calibration of a nine-junction thermopile. For mean temperatures between $-10\:^{o}\textrm{C}$ and $15\:^{o}\textrm{C}$, the thermoelectric sensitivity was measured with an uncertainty of less than $\pm 2\:\%$. Subsequently, temperature differences as low as $10^{-2}\:\textrm{K}$ can be resolved, while the thermometer used for the example calibration was accurate only to $\pm 0.3\:\textrm{K}$. This and higher degrees of accuracy are required in certain research applications, for example to detect heat flux modulations in bifurcating fluidic systems.

==> styles.tex <==


%Colors

%\xdefinecolor{green1}{HTML}{40A562} 
\xdefinecolor{green1}{HTML}{19A347} 
%\xdefinecolor{red1}{HTML}{A54053} D11919
\xdefinecolor{red1}{HTML}{ D11919}
%\xdefinecolor{blue1}{HTML}{4053A5} 2E5CE6
%\xdefinecolor{blue1}{HTML}{2E5CE6}1919FF
\xdefinecolor{blue1}{HTML}{1919FF}
\xdefinecolor{blue2}{HTML}{4083A5}

\xdefinecolor{copper1}{HTML}{B87333}
\xdefinecolor{copperg}{HTML}{527F76}
\xdefinecolor{steel1}{HTML}{8F8FBD}


\xdefinecolor{red1l}{HTML}{F7D4D4}
%TikZ Image Style

\tikzstyle{block} = [rectangle, draw,color=blue1, fill=blue1!10!white!90, line width=1mm, 
    text width=5em,text=black, text centered, rounded corners, minimum height=3em,font=\small]
\tikzstyle{block2} = [rectangle, draw,color=red1, line width=0.25mm, 
   text=black, text centered, rounded corners, minimum height=2em, minimum width =2em,text width=4em,fill=red1!10!white!90,font=\small]% text width=4em,
\tikzstyle{block3} = [rectangle, draw,color=black, fill=white!20, line width=0.25mm, font=\scriptsize,
    text=black, text centered, rounded corners,minimum height=1em, minimum width =2em]%text width=8em,
\tikzstyle{line} = [draw,line width=.25mm, -latex',line join = round]
\tikzstyle{line2} = [draw,line width=.45mm, -latex',line join = round]
\tikzstyle{cloud} = [draw, ellipse,color=blue1,fill=blue1!10!white!90, line width=.45mm,   text centered,text width=6em,  minimum height=2em,text=black,inner sep =0pt]%text width=6em,
\tikzset{dot/.style={circle,fill=#1,inner sep=0,minimum size=4pt}}
\tikzstyle{line3} = [draw,line width=.5mm,line join = round]


%%%%%%% Interrupted Line
\pgfdeclaredecoration{discontinuity}{start}{
  \state{start}[width=0.5\pgfdecoratedinputsegmentremainingdistance-0.5\pgfdecorationsegmentlength,next state=first wave]
  {}
  \state{first wave}[width=\pgfdecorationsegmentlength, next state=second wave]
  {
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfdecorationsegmentamplitude}}
    \pgfpathcurveto
        {\pgfpoint{-0.25*\pgfmetadecorationsegmentlength}{0.75\pgfdecorationsegmentamplitude}}
        {\pgfpoint{-0.25*\pgfmetadecorationsegmentlength}{0.25\pgfdecorationsegmentamplitude}}
        {\pgfpoint{0pt}{0pt}}
    \pgfpathcurveto
        {\pgfpoint{0.25*\pgfmetadecorationsegmentlength}{-0.25\pgfdecorationsegmentamplitude}}
        {\pgfpoint{0.25*\pgfmetadecorationsegmentlength}{-0.75\pgfdecorationsegmentamplitude}}
        {\pgfpoint{0pt}{-\pgfdecorationsegmentamplitude}}
}
\state{second wave}[width=0pt, next state=do nothing]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfdecorationsegmentamplitude}}
    \pgfpathcurveto
        {\pgfpoint{-0.25*\pgfmetadecorationsegmentlength}{0.75\pgfdecorationsegmentamplitude}}
        {\pgfpoint{-0.25*\pgfmetadecorationsegmentlength}{0.25\pgfdecorationsegmentamplitude}}
        {\pgfpoint{0pt}{0pt}}
    \pgfpathcurveto
        {\pgfpoint{0.25*\pgfmetadecorationsegmentlength}{-0.25\pgfdecorationsegmentamplitude}}
        {\pgfpoint{0.25*\pgfmetadecorationsegmentlength}{-0.75\pgfdecorationsegmentamplitude}}
        {\pgfpoint{0pt}{-\pgfdecorationsegmentamplitude}}
    \pgfpathmoveto{\pgfpointorigin}
}
  \state{do nothing}[width=\pgfdecorationsegmentlength,next state=do nothing]{
    \pgfpathlineto{\pgfpointdecoratedinputsegmentlast}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}

%%%USE
%\draw [decoration={%
%        discontinuity,
%        amplitude=5mm, %length of waves
%        segment length=2mm, %space width
%        meta-segment length=2mm}, %amplitude of the wave itself
%    decorate](1,-1) -- (3,-2);


%PGFPLOTSET

\pgfplotsset{
    standard/.style={
%        axis x line=middle,
%        axis y line=middle,
%        enlarge x limits=0.15,
%        enlarge y limits=0.15,
        every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
        every axis y label/.style={at={(current axis.above origin)},anchor=north east}
    }
}

